A primal-dual perspective for distributed TD-learning

The goal of this paper is to investigate distributed temporal difference (TD) learning for a networked multi-agent Markov decision process. The proposed approach is based on distributed optimization algorithms, which can be interpreted as primal-dual Ordinary differential equation (ODE) dynamics subject to null-space constraints. Based on the exponential convergence behavior of the primal-dual ODE dynamics subject to null-space constraints, we examine the behavior of the final iterate in various distributed TD-learning scenarios, considering both constant and diminishing step-sizes and incorporating both i.i.d. and Markovian observation models. Unlike existing methods, the proposed algorithm does not require the assumption that the underlying communication network structure is characterized by a doubly stochastic matrix.

==> app/jcf.tex <==

Number of Jordan blocks corresponding to \(\lambda_i\) is its geometric multiplicity.~\cite{horn2012matrix}


\begin{definition}[Jordan block, Definition 3.1.1 in~\cite{horn2012matrix}]
A Jordan block \(\mJ_k(\lambda) \in \R^{k\times k}\) is an upper triangular matrix of the form
\begin{align*}
    \mJ_k(\lambda) = \begin{bmatrix}
        \lambda & 1 &  &\\
         & \lambda & 1 &\\
         &  & \ddots & \ddots & \\
          &  & & \lambda & 1\\
        & & & &\lambda
    \end{bmatrix} .
\end{align*}
Moreover, A Jordan matrix \(\mJ \in \R^{n\times n}\) is a direct sum of Jordan blocks : 
\begin{align*}
    \mJ= \mJ_{n_1}(\lambda_1) \oplus  \mJ_{n_2}(\lambda_2) \dots \otimes  \mJ_{n_q}(\lambda_q)  
\end{align*}
such that \( \sum_{i=1}^q n_i =n\).
\end{definition}



\begin{theorem}[Theorem 3.1.11 in~\citep{horn2012matrix}]\label{thm:jcf}
    Let \( \mA \in \R^{n\times n}\). There is a non-singular \(S\in \R^{n\times n}\), positive inteqers \(q\) and \(n_1,n_2,\dots,n_q\) such that \(\sum_{i=1}^q n_i  = n\), and \(\lambda_1,\lambda_2,\dots,\lambda_q \in \sC\) such that
    \begin{align*}
        \mA = \mS \mJ  \mS^{-1},
    \end{align*}
    where \(\mJ:=\mathrm{diag}(  \mJ_{n_1}(\lambda_1),  \mJ_{n_2}(\lambda_{2}),\dots, \mJ_{n_q}(\lambda_1))) \). Moreover, \(\mJ\) is unique up to permutation of Jordan blocks.
\end{theorem}

The geometric multiplicity of a given eigenvalue of a Jordan matrix is equal to the number of Jordan blocks corresponding to that eigenvalue. The sum of all the Jordan blocks corresponding to a given eigenvalue is its algebraic multiplicity.

==> app/normalized_lap.tex <==
d\begin{lemma}
    Consider a connected graph \(\gG\) and its laplacian and normalized graph laplacian, \(\mL\) and \(\mL_n\) respectively. For \(\vy\in\R^{d}\), \(\mD^{1/2}\vy\) is in null space of \(\mL_n\) if and only if \(\vy\) is in null space of \(\mL\)
\end{lemma}
\begin{proof}
    We first prove the sufficiency part. If \(\mD^{1/2}\vy\) is in null space of \(\mL_n\), then we have
    \begin{align*}
        &\mD^{-1/2}\mL\mD^{-1/2} (\mD^{1/2}\vy) = \bm{0}_d\\
    \iff & \mL \vy =\bm{0}_d.
    \end{align*}
    Next, we prove the necessary part. If \(\mL\vy=\bm{0}_d\), we have
    \begin{align*}
        \mD^{-1/2}\mL\mD^{-1/2} (\mD^{1/2}\vy)=\mD^{-1/2}\mL\vy = \bm{0}_d.
    \end{align*}
\end{proof}

Consider the update
\begin{align*}
      &\vtheta^i_{k+1}  \\
    =& \vtheta^i_{k}  + \alpha_k \left( \left(\frac{1}{\sqrt{|\gN|_i}}r^i_k + \frac{1}{|\gN|_i}\left(\gamma \bm{\phi}^{\top}(s_{k+1})\vtheta^i_k - \bm{\phi}^{\top}(s_k) \vtheta_k^i\right)\right) \bm{\phi}(s^i_k) \right.\\
    &\left.-\left(\vtheta^i_k-\sum_{j\in \gN_i}\frac{1}{\sqrt{|\gN_i| |\gN_j|} }\vtheta^j_k \right)-\left(\vw^i_k-\sum_{j\in \gN_i}\frac{1}{\sqrt{|\gN_i| |\gN_j|} } \vw^j_k )\right)\right),
\end{align*}

which can be represented in matrix form as

\begin{align*}
    \bar{\vtheta}_k =& \bar{\vtheta}_k+\alpha_k \left(
    \bar{\mD}^{-1}\bar{\mA}\bar{\vtheta}_k+\bar{\mD}^{-1/2}\bar{\vb}-\bar{\mL}_n \bar{\vtheta}_k-\bar{\mL}_n\bar{\vw}_k
    \right) + \alpha_k \bm{\bar{\eps}}(o_k;\bar{\vtheta}_k)\\
    \bar{\vw}_k =& \bar{\vw}_k+\alpha_k \left( \bar{\mL}_n \bar{\vtheta}_k\right)
\end{align*}

where

\begin{align*}
 &   \mD:=\mathrm{diag}(|\gN_1|,|\gN_2|,\dots,|\gN_N|)\in\R^{N\times N}, \quad  \bar{\mD}:=\mD \otimes \mI_q \\
 &     \mL_n = \mD^{-1/2}\mL\mD^{-1/2},\quad   \bar{\mL}_n = \mL_n \otimes \mI_q \in \R^{Nq\times Nq} 
\end{align*}

The goal is to find solution \(\bar{\vtheta}_d,\bar{\vw}_d\) such that 

\begin{align*}
    (\bar{\mD}^{-1}\bar{\mA}-\bar{\mL}_n)\bar{\vtheta}_d-\bar{\mL}_n \bar{\vw}_d &=\bar{\mD}^{-1/2} \bar{\vb}\\
    \bar{\mL}_n\bar{\vtheta}_d &= \bm{0}_{Nq\times Nq}.
\end{align*}

Therefore, we should have 
\begin{align*}
    \bar{\vtheta}_d = (\mD^{1/2}\bm{1}_N)\otimes \vq.
\end{align*}


Now, we will inspect the solution of the update using normalized graph laplacian. First, we can see that

\begin{align*}
   & ( \mD^{1/2} \bm{1}_N \otimes \mI_q)^{\top} \bar{\mL}_n\\ =& \left(\begin{bmatrix}
        \sqrt{|\gN_1|}\mI_q\\
        \sqrt{|\gN_2|}\mI_q\\
        \vdots\\
        \sqrt{|\gN_N|}\mI_q
    \end{bmatrix}\right)^{\top}\begin{bmatrix}
        [\mL_n]_{11}\mI_q & [\mL_n]_{12}\mI_q & \cdots & [\mL_n]_{1N}\mI_q\\
        [\mL_n]_{21}\mI_q & [\mL_n]_{22}\mI_q & \cdots & [\mL_n]_{2N}\mI_q\\
        & & \vdots &\\
        [\mL_n]_{N1}\mI_q & [\mL_n]_{N2}\mI_q & \cdots & [\mL_n]_{NN}\mI_q
    \end{bmatrix}\\ 
    =& \begin{bmatrix}
       \left(\sum_{i=1}^N \sqrt{|\gN_i|} [\mL_n]_{i1}\right) \mI_q & \left(\sum_{i=1}^N \sqrt{|\gN_i|} [\mL_n]_{i2}\right) \mI_q & \cdots &\left(\sum_{i=1}^N \sqrt{|\gN_i|} [\mL_n]_{iN}\right) \mI_q
    \end{bmatrix}\\
    =&\begin{bmatrix}
    \left( \sqrt{|\gN_1|}-\sum_{j\notin[N]\setminus\{1\}} \frac{[\mL]_{j1}}{\sqrt{|\gN_1|}} \right)\mI_q &    \left( \sqrt{\gN_2}-\sum_{j\in[N]\setminus \{2\}} \frac{[\mL]_{j2}}{\sqrt{|\gN_2|}} \right)\mI_q &\cdots &    \left( \sqrt{|\gN_N|}-\sum_{j\in[N]\setminus[N]} \frac{[\mL]_{jN}}{\sqrt{|\gN_N|}} \right)\mI_q
    \end{bmatrix}\\
    =&\bm{0}_{q\times Nq}
\end{align*}

Multiplying \(\) on both equations, we get

\begin{align*}
   & \begin{bmatrix}
        \sqrt{|\gN_1|}\mI_q & \sqrt{|\gN_2|}\mI_q  & \cdots & \sqrt{|\gN_N|}\mI_q 
    \end{bmatrix} (\bar{\mD}^{-1})\bar{\mA}  \vx  = \begin{bmatrix}
        \sqrt{|\gN_1|}\mI_q & \sqrt{|\gN_2|}\mI_q  & \cdots & \sqrt{|\gN_N|}\mI_q 
    \end{bmatrix} \bar{\mD}^{-1/2}\bar{\vb} \\
\iff & \begin{bmatrix}
        \frac{1}{\sqrt{|\gN_1|}}\mI_q & \frac{1}{\sqrt{|\gN_2|}}\mI_q  & \cdots & \frac{1}{\sqrt{|\gN_N|}}\mI_q 
    \end{bmatrix} \bar{\mA}(\mD^{1/2}\bm{1}_N)\otimes \vq   = \sum_{i=1}^N \vb_i \\
\iff& \begin{bmatrix}
        \frac{1}{\sqrt{|\gN_1|}}\mA& \frac{1}{\sqrt{|\gN_2|}}\mA  & \cdots & \frac{1}{\sqrt{|\gN_N|}}\mA 
    \end{bmatrix} \begin{bmatrix}
        \sqrt{|\gN_1|}\vq\\
        \sqrt{|\gN_2|}\vq\\
        \vdots\\
        \sqrt{|\gN_N|}\vq
    \end{bmatrix} = \sum_{i=1}^N \vb_i \\
\iff&   \sum_{i=1}^N \mA \vq    =\sum_{i=1}^N \vb_i\\
\iff&   \vq = \frac{\sum_{i=1}^N \vb_i }{N} \mA^{-1}.
\end{align*}

To measure the error with the original solution, we need to multiply 

\begin{align*}
    \left\|(\mD^{-1/2}\otimes \mI_q)(\bar{\vtheta}_k-\bar{\vtheta}_d)\right\|&=\left\|(\mD^{-1/2}\otimes \mI_q)\bar{\vtheta}_k-(\mD^{-1/2}\otimes \mI_q)((\mD^{1/2}\bm{1}_N)\otimes \vq)\right\|_2\\
    &=\left\| (\mD^{-1/2}\otimes \mI_q)\bar{\vtheta}_k- \bm{1}_N\otimes \vq \right\|_2.
\end{align*}


Note that

\begin{align*}
     (\mD^{-1/2}\otimes \mI_q)\bar{\vtheta}_k = \begin{bmatrix}
         \frac{1}{\sqrt{|\gN_1|}}\vtheta^1_k\\
         \frac{1}{\sqrt{|\gN_2|}}\vtheta^1_k\\
         \vdots\\
         \frac{1}{\sqrt{|\gN_N|}}\vtheta^N_k
     \end{bmatrix} .
\end{align*}

==> app/projection.tex <==
Consider the following matrix :
\begin{align*}
    \bar{\mE}:=\begin{bmatrix}
        \bar{\mA} & - \bar{\mL}\\
        \bar{\mL} & \bm{0}_{Nq \times Nq}
    \end{bmatrix},
\end{align*}

The projection onto \(\mathrm{Im}(\bar{\mE}^{\top})\) is defined as
\begin{align*}
    \mP =   \begin{bmatrix}
        \mI_{Nq} & \bm{0}_{Nq\times Nq}\\
        \bm{0}_{Nq \times Nq} & \mL\mL^{\dagger}
    \end{bmatrix},
\end{align*}

because \(\mP^2=\mP\) and 
\begin{align*}
    \mathrm{Ker}(\mP) &=  \left\{  \begin{bmatrix}\bm{0}_{Nq} \\ \vy \end{bmatrix} \middle | \vy \in \mathrm{Ker}(\bar{\mL}) \right\}\\
    \mathrm{Im}(\mP) &= \left\{ \begin{bmatrix}
        \vx\\
        \vy
    \end{bmatrix} \middle | \vx\in\R^d,\;\vy \in \mathrm{Im}(\mL) \right\},
\end{align*}
hence, it becomes projection on to \(\mathrm{Im}(\mE)\). 

For \(\vx\in\R^d ,\vy\in \mathrm{Im}(\mL)\), have

\begin{align*}
    \bar{\mA}\vw-\bar{\mL}\vv= \vx\\
    \bar{\mL}\vw = \bar{\mL}\vz
\end{align*}
for some \(\vz\in\R^{Nq}\). We can choose \(\vw=\vz,\) and letting \(\vv=\bm{1}_{N}\otimes \vq\) ofr \(\vq \in \R^{q}\).



Consider


\begin{align*}
\begin{bmatrix}
    \bar{\vtheta}_k\\
    \bar{\tilde{\vw}}
\end{bmatrix}^{\top}
\begin{bmatrix}
    \bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL} & \bm{0}_{Nq\times Nq}\\
    \bm{0}_{Nq \times Nq} & -2\bar{\mL}-2\alpha \mU\mU^{\top}
\end{bmatrix}
\begin{bmatrix}
    \bar{\vtheta}_k\\
    \bar{\tilde{\vw}}
\end{bmatrix}
= -\lambda_{\min} \left\| \bar{\vtheta}_k \right\|_2^2
-\min(\bar{\mL},\alpha)\left\| \bar{\vw}_k \right\|_2^2
\end{align*}


Given an eigenvalue \(\lambda\), we have
\begin{align*}
    &\bar{\mA}\vx - \bar{\mL}\vy = \lambda \vx\\
    & \bar{\mL}\vx = \lambda \vy
\end{align*}

We have
\begin{align*}
  \bar{\mA} \vx - \frac{1}{\lambda} \bar{\mL}^2 \vx = \lambda \vx
\end{align*}

==> app/pseudo_inverse.tex <==
The projection onto the row space , which is orthogonal to the null space is

\begin{align*}
    \mA^{\dagger}\mA
\end{align*}

The null space of projection operator is

\begin{align*}
&    \mA^{\dagger}\mA \vx =0\\
\rightarrow & \mA \mA^{\dagger}\mA \vx =0 \\
\rightarrow & \mA\vx =0 .
\end{align*}

Hence, \(\vx\in \mathrm{Ker}(\mA^{\dagger}\mA)\) then, \(\vx \in \mathrm{Ker}(\mA)\). The converse is trivial. Moreover, if \( \vx \in \mathrm{Ker}(\mA^{\top})\), then 



\subsection{Kernel and image}

Consider the following matrix:
\begin{align*}
    \mE:=\begin{bmatrix}
        \mA & - \mL\\
        \mL & \bm{0}_{d \times d}
    \end{bmatrix}.
\end{align*}

Then, 
\begin{align*}
    \mathrm{Ker}(\mE) = \left\{\begin{bmatrix}
                            \bm{0}_{Nq}\\
                            \bm{1}_{N}\otimes \vv
                        \end{bmatrix} \middle| \vv \in \R^q\right\}
\end{align*}

Note that 
\begin{align*}
    \mathrm{Ker}(\mE)= \mathrm{Ker}(\mE^{\top}),
\end{align*}
which also implies
\begin{align*}
    \mathrm{Img}(\mE)=\mathrm{Img}(\mE^{\top}).
\end{align*}

Moreover, let
\begin{align*}
    \mE:= \mU \bm{\Sigma} \mV^{\top},
\end{align*}
where \(\mathrm{rank}(\mE)=r\). Then,

\begin{align*}
&    \mE^{\top}\mE \mV= \begin{bmatrix}
                            \mV_{1:r} &
                            \mV_{r+1:n}
                       \end{bmatrix}
                       \begin{bmatrix}
                           \bm{\Sigma}^2_+ &  \bm{0}_{{r}\times (n-r)}\\
                            \bm{0}_{(n-r)\times r}& \bm{0}_{ (n-r) \times (n-r)}
                       \end{bmatrix}\\
\iff & \begin{bmatrix}
        \mE^{\top}\mE \mV_{1:r} &
        \mE^{\top}\mE \mV_{r+1:n}
        \end{bmatrix}=
        \begin{bmatrix}
            \mV_{1:r} \bm{\Sigma}^2_+ & \bm{0}_{n:n-r}
        \end{bmatrix}\\
\iff & \mE^{\top}\mE \mV_i = \sigma_1^2 \mV_i,\quad 1 \leq i \leq r\\
     & \mE^{\top}\mE \mV_i = \bm{0}_n,\quad r+1 \leq i \leq n.
\end{align*}

Therefore, \(\mV_i\in \mathrm{Img}(\mE^{\top})\). Suppose we have

\begin{align*}
 \mP \mB + \mB^{\top}\mP = -\mI,
\end{align*}

where 

\begin{align*}
    \mB := \mE- \alpha \mT_{1:q} \mS_{1:q}^{\top},
\end{align*}

We have
\begin{align*}
    \mP \mE + \mE^{\top}\mP =-\mI +\alpha \mP \mT_{1:q}\mS^{\top}_{1:q}+\alpha \mS_{1:q}\mT^{\top}_{1:q}\mP.
\end{align*}

Multiplying the projection operator, we have

\begin{align*}
    \mE\mE^{\dagger} \mP\mE+ \mE\mE^{\dagger} \mE^{\top}\mP= - \mE\mE^{\dagger}+\alpha ( \mE\mE^{\dagger}\mP\mT_{1:q}\mS^{\top}_{1:q}+\alpha  \mE\mE^{\dagger}\mS_{1:q}\mT^{\top}_{1:q}\mP) 
\end{align*}


Note that

\begin{align*}
    \mE\mE^{\dagger}\mE^{\top}=&\mU \bm{\Sigma} \mV^{\top} \mV \bm{\Sigma}_+^{-1} \mU^{\top}\mV \bm{\Sigma}\mU^{\top}\\
    =&\mU \begin{bmatrix}
        \mI_{r} & \bm{0}_{r\times(n-r)}\\
        \bm{0}_{( n-r) \times r} & \bm{0}_{(n-r)\times(n-r)}
    \end{bmatrix} \mU^{\top}\mV\bm{\Sigma}\mU^{\top}\\
    =& \mU_{1:r} \mU_{1:r}^{\top} \mV \bm{\Sigma} \mU^{\top}
\end{align*}






\subsection{Lower bound on minimum singualr value}


Let 

\begin{align*}
    \mE :=  \begin{bmatrix}
 \bar{\mA}-\Bar{\mL} & -\bar{\mL}\\
 \bar{\mL} & \bm{0}_{Nq \times Nq}
 \end{bmatrix}
\end{align*}
\begin{align*}
 \sigma_{\min}^+\left( \mE \right) &= \min_{ \substack{\left\|\vv \right\|_2 =1\\
 \vv \notin \mathrm{Ker}(\mE)
 }}
 \left\|
 \begin{bmatrix}
 \bar{\mA}-\Bar{\mL} & -\bar{\mL}\\
 \bar{\mL} & \bm{0}_{Nq \times Nq}
 \end{bmatrix} \vv
  \right\|_2 \\
&\geq \min_{\substack{\left\| \vv\right\|_2=1\\\vv\notin\mathrm{Ker}(\mE)}} \max \{\left\|\mE_1 \vv \right\|,\left\| \mE_2\vv\right\|_2  \}\\
&\geq 
\max\left\{
\min_{ \substack{\left\|\vv \right\|_2 =1\\
 \vv \notin \mathrm{Ker}(\mE)
 }}\left\|\begin{bmatrix}
    \bar{\mA}-\bar{\mL} & -\bar{\mL}
\end{bmatrix}\vv\right\|_2,
\min_{ \substack{\left\|\vv \right\|_2 =1\\
 \vv \notin \mathrm{Ker}(\mE)
 }}\left\|\begin{bmatrix}
    \bar{\mL} & \bm{0}_{Nq\times Nq}
\end{bmatrix}\vv\right\|_2,
\right\}\\
&\geq
\min\left\{
\min_{ \substack{\left\|\vv \right\|_2=1\\ \vv \notin \mathrm{Ker}(\mE_1)}} \left\| \mE_1\vv \right\|_2,
\min_{\substack{\left\|\vv\right\|_2=1\\ \vv \notin \mathrm{Ker}(\mE_2)}}\left\|\mE_2 \right\|_2
\right\}
\end{align*}

The last inequatliy follows since if \(\vv \notin \mathrm{Ker}(\mE_1) \) and \(\vv \in \mathrm{Ker}(\mE_2)\), then

\begin{align*}
    \max\left\{
\min_{ \substack{\left\|\vv \right\|_2 =1\\
 \vv \notin \mathrm{Ker}(\mE)
 }}\left\|\begin{bmatrix}
    \bar{\mA}-\bar{\mL} & -\bar{\mL}
\end{bmatrix}\vv\right\|_2,
\min_{ \substack{\left\|\vv \right\|_2 =1\\
 \vv \notin \mathrm{Ker}(\mE)
 }}\left\|\begin{bmatrix}
    \bar{\mL} & \bm{0}_{Nq\times Nq}
\end{bmatrix}\vv\right\|_2,
\right\}= \min_{ \substack{\left\|\vv \right\|_2=1\\\vv \in \mathrm{Ker}(\mE_2)\\\vv \notin \mathrm{Ker}(\mE_1)}} \left\| \mE_1 \vv \right\|_2 \geq \min_{\substack{\left\|\vv\right\|_2=1\\ \vv\notin\mathrm{Ker}(\mE_1)}} \left\| \mE_1 \vv \right\|_2.
\end{align*}


Hence, it is enough to lower bound each minimum singular values. Therefore, we need lower bound minimum non-zero singular value of \(\mE_1\).

\begin{align*}
    \sigma_{\min}^+ (\mE_1) =& \min_{\substack{\left\|\vv_1 \right\|_2=1\\\vv\notin\mathrm{Ker}(\mE_1)}} \left\| \mE_1 \vv \right\|_2 \\
    =& \min_{\substack{\left\|\vv_1 \right\|_2=1\\\vv\notin\mathrm{Ker}(\mE_1^{\top})}} \left\|
    \begin{bmatrix}
        (\bar{\mA}-\bar{\mL})^{\top}\vv\\
         -\bar{\mL}\vv
    \end{bmatrix}
    \right\|_2\\
    \geq &\min_{\substack{\left\|\vv_1 \right\|_2=1\\\vv\notin\mathrm{Ker}(\mE_1^{\top})}} 
    \max \left\{ \left\|(\bar{\mA}-\bar{\mL})^{\top}\vv \right\|_2, \left\|\bar{\mL}\vv\right\|_2 \right\}\\
    \geq &  \max\left\{ \min_{\substack{\left\|\vv_1 \right\|_2=1\\\vv\notin\mathrm{Ker}(\mE_1^{\top})}} \left\| (\bar{\mA}-\bar{\mL})^{\top}\vv\right\|_2,\min_{\substack{\left\|\vv_1 \right\|_2=1\\\vv\notin\mathrm{Ker}(\mE_1^{\top})}} \left\| \bar{\mL}\vv\right\|_2   \right\}\\
    \geq & \min \left\{
    \min_{\substack{\left\|\vv\right\|_2=1\\\vv\notin \mathrm{Ker}(\bar{\mA}-\bar{\mL})}}\left\| \right(\bar{\mA}-\bar{\mL})\vv\|_2,\min_{\substack{\left\| \vv\right\|_2=1\\\vv\notin\mathrm{Ker}(\bar{\mL})}}\left\|\bar{\mL}\vv\right\|_2
    \right\}.
\end{align*}
Hence, we need a lowe bound on the minimum singular value of \(\bar{\mA}-\bar{\mL}\). From Wely's inequaltiy of singular value version, we have

\begin{align*}
    \sigma^+_{\min}(\bar{\mA}-\bar{\mL}) &= \sigma_{\min}(\bar{\mA}-\bar{\mL})\\
    &\geq -\left\|\bar{\mL}\right\|_2 +\sigma_n(\bar{\mA})
\end{align*}

==> app/saddlepoint_matrix.tex <==
The matrix
\begin{align*}
    \begin{bmatrix}
        \mA & \mB^{\top}\\
        -\mB & \bm{0}
    \end{bmatrix}
\end{align*}
is called a saddle point matrix~\citep{benzi2005numerical}.~\cite{qu2018exponential} found Lyapunov solution when \(\mB\) is non-singular. Following the spirit of~\cite{qu2018exponential}, let the solution of the Lyapunov equation

\begin{align*}
    \mP:= \begin{bmatrix}
        c\mI & \mL\\
        \mL & c\mI
    \end{bmatrix}.
\end{align*}

If \(c>2 \kappa_L^2\), considering the Schur complement we have

\begin{align*}
    \begin{bmatrix}
        \frac{c}{2}\mI & \bm{0}\\
        \bm{0} & \frac{c}{2}\mI
    \end{bmatrix}
    \prec \mP
    \prec
    \begin{bmatrix}
        2c \mI &\bm{0}\\
        \bm{0} & 2c \mI
    \end{bmatrix}
\end{align*}
% Considering the Schur complement, for the matrix to be positive definite, we should have

% \begin{align*}
%     &c^2\mI-\mL^2 \succ 0\\
%     \iff & c^2 > \kappa_L^2
% \end{align*}


Now, consider 

\begin{align*}   
    \begin{bmatrix}
        c\mI & \mL\\
        \mL & c\mI
    \end{bmatrix}
    \begin{bmatrix}
        \bar{\mA}-\bar{\mL} & - \bar{\mL}\\
        \bar{\mL} & \bm{0}
    \end{bmatrix}
    =\begin{bmatrix}  
    c(\bar{\mA}-\bar{\mL})+\bar{\mL}^2 & -c\bar{\mL}\\
    \bar{\mL}\bar{\mA}-\bar{\mL}^2+c\bar{\mL} & -\bar{\mL}^2
    \end{bmatrix},
\end{align*}

which results to

\begin{align*}
    \begin{bmatrix}
        c(\bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL})+2\bar{\mL}^2
        &(\bar{\mA}^{\top}-\bar{\mL})\bar{\mL}\\
        \bar{\mL}(\bar{\mA}-\bar{\mL}) &-2\bar{\mL}^2
    \end{bmatrix}.
\end{align*}


Considering the iterate \(\tilde{\vw}=\bar{\mL}\bar{\mL}^{\dagger} \), we have

\begin{align*}
   & \begin{bmatrix}
        \bar{\vtheta}_k\\
        \tilde{\vw}
    \end{bmatrix}^{\top}
        \begin{bmatrix}
        c(\bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL})
        &(\bar{\mA}^{\top}-\bar{\mL})\bar{\mL}\\
        \bar{\mL}(\bar{\mA}-\bar{\mL}) &-2\bar{\mL}^2
    \end{bmatrix}
    \begin{bmatrix}
        \bar{\vtheta}_k\\
        \tilde{\vw}_k
    \end{bmatrix}\\
    =&\bar{\vtheta}_k^{\top}(c(\bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL}))\bar{\vtheta}_k
    +\bar{\vtheta}_k^{\top}(\bar{\mA}^{\top}-\bar{\mL})\bar{\mL}\tilde{\vw}_k\\
    +& \tilde{\vw}_k^{\top}\bar{\mL}(\bar{\mA}-\bar{\mL})\bar{\vtheta}_k-2\tilde{\vw}_k^{\top} \bar{\mL}^2\tilde{\vw}_k\\
    =&\bar{\vtheta}_k^{\top}(c(\bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL}))\bar{\vtheta}_k
    +\bar{\vtheta}_k(\bar{\mA}^{\top}-\bar{\mL})\tilde{\vw}_k\\
    +& \bar{\vw}_k^{\top}(\bar{\mA}-\bar{\mL})\bar{\vtheta}_k -2 \left\| \tilde{\vw}_k \right\|_2\\
    =&
    \begin{bmatrix}
        \bar{\vtheta}_k\\
        \bar{\mL}\bar{\vw}_k
    \end{bmatrix}^{\top}
    \begin{bmatrix}
        c(\bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL})+\bar{\mL}^2 & \bar{\mA}^{\top}-\bar{\mL}\\
        \bar{\mA}-\bar{\mL} & -2 \mI
    \end{bmatrix}
        \begin{bmatrix}
        \bar{\vtheta}_k\\
        \bar{\mL}\bar{\vw}_k
    \end{bmatrix}
\end{align*}
Hence it is enough to bound the above matrix.


Consider:


\begin{align*}
\begin{bmatrix}
        (c\kappa_1+b+\kappa_2) \mI & \bar{\mA}^{\top}-\bar{\mL}\\
    \bar{\mA}-\bar{\mL} & (-2+b)\mI
\end{bmatrix},
\end{align*}

where \( \kappa_1 = \lambda_{\max}(\bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL})<0\) and \(0<b<2\). Using the Schur complement argument, we need

\begin{align*}
    &(c\kappa_1+\kappa_2+b)\mI+\frac{1}{2-b}(\bar{\mA}^{\top}-\bar{\mL})(\bar{\mA}-\bar{\mL}) \prec 0\\
    \iff& (c\kappa_1+\kappa_2+b)+\frac{1}{2-b}\kappa_3<0.
\end{align*}

We need

\begin{align*}
    c> \frac{\kappa_3}{-\kappa_1(2-b)}-\frac{1+\kappa_2}{\kappa_1 b}=\frac{\left\|\bar{\mA}^{\top}-\bar{\mL} \right\|_2}{-\lambda_{\max}(\bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL})}
    +\frac{1+\left\| \bar{\mL} \right\|^2_2}{\lambda_{\max}(\bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL})}.
\end{align*}

It suffices to choose 
\begin{align*}
    c = 2\frac{\left\| \bar{\mA}\right\|_2+\left\| \bar{\mL} \right\|_2}{-\lambda_{\max}(\bar{\mA}+\bar{\mA}^{\top})}
\end{align*}


Note that 
\begin{align*}
    \left\| \bar{\mL}^{\dagger}\bar{\mL}\bar{\vw}_k\right\|_2 \leq \left\| \bar{\mL}^{\dagger} \right\|_2 \left\|\bar{\mL}\bar{\vw}\right\|_2
\end{align*}




Suppose we are interested only in the range space solution, then
\begin{align*}
 \Tilde{\vx}_k:=   \mA\mA^{\dagger} \vx_k,
\end{align*}
we have
\begin{align*}
    \tilde{\vx}_k =\tilde{\vx}_k+\alpha_k \mA \vx_k+ \mA\mA^{\dagger}\bm{\eps}_k.
\end{align*}

Note that 
\begin{align}
 & \E\left[V(\tilde{\vx}_{k+1})\right] \nonumber   \\
=& \E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k) \right]+\E\left[ 2\tilde{\vx}_k^{\top}\mP \tilde{\vx}_{k+1} \right] -2 \E\left[V(\tilde{\vx}_k)\right] \nonumber \\
=& \E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k) \right]+\E \left[ 2\tilde{\vx}_k^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k)\right] \nonumber\\
=&\E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k ) \right]+\E\left[2\tilde{\vx}_k^{\top}\mP(\tilde{\vx}_{k+1}-\tilde{\vx}_k-\alpha_k\mA \tilde{\vx}_k) \right]+2\alpha_k \E\left[ \tilde{\vx}_k^{\top} \mP \mA \tilde{\vx}_k \right]  \nonumber\\
\leq &\E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k ) \right]+\E\left[2\tilde{\vx}_k^{\top}\mP(\tilde{\vx}_{k+1}-\tilde{\vx}_k-\alpha_k\mA \tilde{\vx}_k) \right]+2\alpha_k \left(
-\left\|\tilde{\vtheta}_k \right\|^2_2-\left\|\bar{\mL}\bar{\vw}_k \right\|_2^2
\right) \nonumber\\
\leq & \E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k ) \right]+2\alpha_k \left(
-\left\|\tilde{\vtheta}_k \right\|^2_2-\sigma_{\min}(\bar{\mL})^+\left\|\tilde{\vw}_k\right\|_2^2
\right) \nonumber\\
\leq & \E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k ) \right]-2\alpha_k \min\{1,\sigma_{\min}(\bar{\mL})^+ \} \left\|\tilde{\vx}_k\right\|_2^2.
\end{align}


\subsection{Analysis of Algroithm 2}

Consider the following matrix:

\begin{align*}
    \begin{bmatrix}
    \bar{\mA}-\bar{\mL} & \bm{0}_{Nq \times Nq} & \bm{0}_{Nq \times Nq}\\
   \eta \bar{\mI}_{Nq} & -\eta\bar{\mI}_{Nq}-\eta\bar{\mL} & -\bar{\mL}\\
    \bm{0}_{Nq\times Nq} & \bar{\mL} & \bm{0}_{Nq \times Nq}
\end{bmatrix}
\end{align*}


With small enough \(\eta\), we will have

\begin{align*}
    c\begin{bmatrix}
    \bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL} &\mI\\
    \mI & -2\mI-2\bar{\mL}
    \end{bmatrix}
    +2\begin{bmatrix}
        \bm{0}&\bm{0}\\
        \bm{0}&2\bar{\mL}^2 
    \end{bmatrix}
    \prec 0
\end{align*}

     
\begin{align*}
    \mP := \begin{bmatrix}
      c  \mI_{Nq\times Nq} & \bm{0}_{Nq\times Nq} &
            \bm{0}_{Nq \times Nq}\\
\bm{0}_{Nq \times Nq} & c \mI_{Nq\times Nq} & \bar{\mL}\\
\bm{0}_{Nq \times Nq} & \bar{\mL} & c \mI_{Nq \times Nq}
    \end{bmatrix}
\end{align*}

For the matrix to be postiive definite, we need

\begin{align*}
    c\mI_{2Nq\times Nq}-\frac{1}{c}\begin{bmatrix}
        \bm{0}&\bm{0}\\
        \bm{0} & \bar{\mL}^2
    \end{bmatrix} \prec 0 \iff c > \kappa_2,
\end{align*}
where \(\kappa_2 = \lambda_{\max}(\bar{\mL})\). To make \(\frac{c}{2}\prec \mP \prec 2c\mI\), we need
\begin{align*}
    c > 4 \kappa_2.
\end{align*}

Now, we have

\begin{align*}
    \mP \begin{bmatrix}
    \bar{\mA}-\bar{\mL} & \bm{0}_{Nq \times Nq} & \bm{0}_{Nq \times Nq}\\
    \eta\bar{\mI}_{Nq} & -\eta\bar{\mI}_{Nq}-\eta\bar{\mL} & -\bar{\mL}\\
    \bm{0}_{Nq\times Nq} & \bar{\mL} & \bm{0}_{Nq \times Nq}
\end{bmatrix} = \begin{bmatrix}
    c(\bar{\mA}-\bar{\mL}) & \bm{0}_{Nq \times Nq} &\bm{0}_{Nq\times Nq} \\
    c\eta\bar{\mI}_{Nq} & -c\eta \bar{\mI}_{Nq}-c\eta\bar{\mL}+\bar{\mL}^2 & -c\bar{\mL}\\
    \eta \bar{\mL} & -\eta\bar{\mL}-\eta\bar{\mL}^2+c\bar{\mL} & -\bar{\mL}^2
\end{bmatrix}
\end{align*}

The result of Lyapunov equation becomes

\begin{align*}
    \begin{bmatrix}
        c(\bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL}) & c\eta\bar{\mI}_{Nq} & \eta\bar{\mL}\\
        c\eta\bar{\mI} & -2c\eta\bar{\mI}_{Nq}-2c\eta\bar{\mL}+2\bar{\mL}^2 & -2\eta\bar{\mL}-2\eta\bar{\mL}^2 \\
        \eta\bar{\mL} & -2\eta\bar{\mL}-2\eta\bar{\mL}^2 & -2\bar{\mL}^2
    \end{bmatrix} .
\end{align*}

After multipyling the coordinate transofrmation, it would be suffice to bound 
\begin{align*}
  \begin{bmatrix}
        c(\bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL}) & c\eta\bar{\mI}_{Nq} & \eta\bar{\mI}\\
        c\eta\bar{\mI} & -2c\eta\bar{\mI}_{Nq}-2c\eta\bar{\mL}+2\bar{\mL}^2 & -2\eta\mI-2\eta\bar{\mL} \\
        \eta\mI & -2\eta\mI-2\eta\bar{\mL} & -2\mI
    \end{bmatrix} .
\end{align*}


We first need to choose small enough \(\eta\) such that

\begin{align*}
&    \begin{bmatrix}
        \bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL} & \eta \mI\\
        \eta \mI & -2\eta \mI
    \end{bmatrix}\prec -\eta \mI .
\end{align*}

Considering the Schur complement, we would need

\begin{align*}
    \kappa_1 +\eta + \eta< 0 \iff 2\eta  <-\kappa_1,
\end{align*}

where \(\kappa_1= \lambda_{\max}(\bar{\mA}+\bar{\mA}^{\top})\), hence we need
\begin{align*}
    \eta < \frac{-\kappa_1}{2}.
\end{align*}

If \(c\eta >2\kappa_2^2+2\), we get

\begin{align*}
    \begin{bmatrix}
        c(\bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL}) & c\eta \mI\\
        c\eta \mI & -2c\eta\mI-2c\eta\bar{\mL}
    \end{bmatrix}
    +\begin{bmatrix}
        \bm{0} & \bm{0}\\
        \bm{0} & 2\bar{\mL}^2
    \end{bmatrix} \prec -c\eta\mI + 2\kappa_2^2 \mI \prec -2\mI
\end{align*}


Therefore, we now have

\begin{align*}
  &\begin{bmatrix}
        c(\bar{\mA}+\bar{\mA}^{\top}-2\bar{\mL}) & c\eta\bar{\mI}_{Nq} & \eta\bar{\mI}\\
        c\eta\bar{\mI} & -2c\eta\bar{\mI}_{Nq}-2c\eta\bar{\mL}+2\bar{\mL}^2 & -2\eta\mI-2\eta\bar{\mL} \\
        \eta\mI & -2\eta\mI-2\eta\bar{\mL} & -2\mI
    \end{bmatrix} \\
\prec &
  \begin{bmatrix}
        -2\mI & \bm{0} & \eta\bar{\mI}\\
        \bm{0} & -2\mI & -2\eta\mI-2\eta\bar{\mL} \\
        \eta\mI & -2\eta\mI-2\eta\bar{\mL} & -2\mI
    \end{bmatrix} .
\end{align*}

To make the above matrix has maximum eigenvalue -1, we need

\begin{align*}
&    -\mI + \begin{bmatrix}
        \eta^2 \mI & -2\eta^2(\mI+\bar{\mL})\\
        -2\eta^2(\mI+\bar{\mL}) & 4\eta^2 (\mI+\bar{\mL})^2
    \end{bmatrix} \prec 0\\
&\iff -1+ \eta^2 \lambda<0 \iff \eta < \frac{1}{\sqrt{\lambda}},
\end{align*}
where \(\lambda\) is the maxinum eigenvalue of the above matrix. We can get the lower bound on the maximum eigenvalue of the matrix. The eigenvalues should satisfity the folloiwng equations:

\begin{align*}
    \vx-2(\mI+\bar{\mL})\vy &= \lambda \vx\\
    -2(\mI+\bar{\mL})\vx+4(\mI+\bar{\mL})^2\vy &=\lambda \vy,
\end{align*}

which is satisfied if

\begin{align*}
    &2(\mI+\bar{\mL})\vx =-\vy,
\end{align*}
and
\begin{align*}
    (5\mI+2\bar{\mL}+\bar{\mL}^2) \vy= \lambda \vy
\end{align*}

Hence, \(\lambda \geq 5\). Therefore, we need \(\eta < \frac{1}{5}\). Therefore, selecting \(\eta = \min\left\{\frac{1}{10},-\frac{\kappa_1}{2}\right\}\), we need

\begin{align*}
    c> \max\left\{ (\kappa_2^2+2) \max\left\{10,\frac{2}{\kappa_1}\right\},4\kappa_2 \right\}.
\end{align*}

Therefore we can choose \(c=2\max\left\{ (\kappa_2^2+2) \max\left\{10,\frac{2}{\kappa_1}\right\},4\kappa_2\right\}\).

Hence, we have

\begin{align*}
   &  \lambda_{\max}(\mP) < 2 \kappa_2^2 \max\left\{ 10,\frac{2}{\kappa_1} \right\}\\
   & \lambda_{\min}(\mP) > \max\left\{ \frac{2\kappa_2^2+4}{\kappa_1}, 4^{1/3}\kappa_2^{2/3}\right\}.
\end{align*}



==> markov_noise.tex <==
The projected iterate becomes


We need to bound

\begin{align*}
    \E\left[ \mA\mA^{\dagger}\vx_k^{\top} \bar{\mA}^{\top}\bm{\eps}_k \right]
\end{align*}


We consider projecting on to the bounded set:

\begin{align*}
    \begin{bmatrix}
        \bar{\vtheta}_{k+1}\\
        \bar{\vw}_{k+1}
    \end{bmatrix}
    =& \mathrm{Proj}_{R}\left(
    \begin{bmatrix}
    \bar{\vtheta}_k\\
    \bar{\vw}_k
\end{bmatrix} 
+\alpha_k \left(
\begin{bmatrix}
    \bar{\mA}-\bar{\mL} & -\bar{\mL}\\
    \bar{\mL} & \bm{0}_{Nq\times Nq}
\end{bmatrix}
\begin{bmatrix}
    \bar{\vtheta}_k\\
    \bar{\vw}_k
\end{bmatrix}
+\begin{bmatrix}
    \bar{\vb}\\
    \bm{0}_{Nq}
\end{bmatrix}
+  \bar{\bm{\eps}}_k \right)\right)
\end{align*}

Why do we need projection? Guaranteeing boundedness of iterate under the Markovian noise does not seem to be possible?


We first need to establish the following bound:

\begin{align*}
    \left\lVert \tilde{\vx}_{k+1}-\tilde{\vx}_k \right\rVert_2^2 =& \left\lVert \mathrm{Proj}\left(\vx_k+\alpha_k \bar{\mE}\tilde{\vx}_k+\bm{\eps}_k\right) 
    -\mathrm{Proj}(\tilde{\vx}_k)\right\rVert_2^2\\
    \leq & \alpha_k^2\left\| \bar{\mE}\tilde{\vx}_k+\bm{\eps}_k\right\|^2_2 \\
    \leq & \alpha_k^2 G^2.
\end{align*}

We have

\begin{align*}
    \left\| \tilde{\vx}_{k}-\tilde{\vx}_{k-\tau} \right\|_2 \leq \sum_{i=k-\tau}^{k-1} \left\| \tilde{\vx}_{i+1}-\tilde{\vx}_i \right\|_2 \leq \sum^{k-1}_{i=k-\tau} \alpha_k G = G \sum^{k-1}_{i=k-\tau} \alpha_k 
\end{align*}

% Consider the weighted norm

% \begin{align*}
%    \sum_{j=1}^{|\gS|} [\mD^{\pi}(\gamma \mP^{\pi} -\mI)]_{ij} = 
%   ( -d_{ii}+\gamma[p]_{ij})+\gamma ( d_{ii}(1-p_{ii}))
%   =d_{ii}(-1+\gamma(1-p_{ii}))+\gamma[p]_{ii}
% \end{align*}

From the control coupling lemma, we have

\begin{align}
    \E\left[ \tilde{\vx}_{t-\tau}^{\prime\top}\bar{\mE}\bm{\eps}(\bar{\vx}_{k-\tau}^{\prime},\bar{\xi}_k^{\prime}) \right] = 0 .\label{eq:lagged_cross_term}
\end{align}

Since \(\bar{\vx}_{k-\tau}\to s_{t-\tau}\to s_t \to O_t\) forms a Markov chain, from Lemma~\ref{lem:control_copuling}, we have
\begin{align*}
    \E[ \tilde{\vx}^{\top}_{k-\tau}\bar{\mE}\bm{\eps}(\bar{\vx}_{k-\tau},\bar{\xi}_{k})   ] \leq 2(2G^2) m \rho^{\tau}.
\end{align*}

From Lipschitzness, we get


\begin{align*}
    \E[\tilde{\vx}_k^{\top} \bar{\mE} \bm{\eps}(\vx_k,\bar{\xi}_k)-\tilde{\vx}_{k-\tau}^{\top} \bar{\mE} \bm{\eps}(\vx_{k-\tau},\bar{\xi}_k)] \leq G \left\| \tilde{\vx}_k-\tilde{\vx}_{k-\tau} \right\|_2\leq G^2 \sum^{k-1}_{i=k-\tau} \alpha_i,
\end{align*}

which results to for \(k \geq \tau^{\mathrm{mix}}(\alpha_T)\),

\begin{align*}
    \E[\tilde{\vx}_k^{\top}\bar{\mE}\bm{\eps}(\bar{\vx}_k,\bar{\xi}_k)] &\leq 4G^2 m \rho^{\tau^{\mathrm{mix}}(\alpha_T)} +G^2 \sum^{k-1}_{i=k-\tau^{\mathrm{mix}}(\alpha_T)}\alpha_i\\
    &\leq 4G^2 \alpha_T+G^2 \tau(\alpha_T) \alpha_{k-\tau(\alpha_T)}\\
    &\leq 8G^2 \tau(\alpha_T) \alpha_{k-\tau(\alpha_T)} .
\end{align*}
and for \(k \leq \tau(\alpha_T)\),
\begin{align*}
        \E[\tilde{\vx}_k^{\top}\bar{\mE}\bm{\eps}(\bar{\vx}_k,\bar{\xi}_k)] \leq G^2 \sum^{k-1}_{i=0} \alpha_i
        \leq G^2 h_1 \log \left(\frac{k-1+h_2}{h_2}\right)+G^2\frac{h_1}{h_2}
\end{align*}

\begin{lemma}[Bound on the cross term]
    \begin{align*}
        \E[\tilde{\vx}_k^{\top}\bar{\mE}\bm{\eps}(\tilde{\vx}_k,\bar{\xi}_k)] \leq \tau(\alpha_T)
    \end{align*}
\end{lemma}



\begin{theorem}
    With \( K_3h_1 = 2\), and \(h_2>2\), we have
    \begin{align*}
        \E\left[\left\|\bar{\vtheta}_T  - \bm{1}_{N}\otimes \vtheta_c   \right\|\right] \leq \tilde{O}\left( \frac{1}{T} \right) .
    \end{align*}
\end{theorem}
\begin{proof}
    
The recursion with Markovian noise term becomes

\begin{align*}
   & \E[V(\tilde{\vx}_{k+1})] \\
   \leq & \left(1-\frac{K_3h_1}{k+h_2}\right)\E[V(\tilde{\vx}_k)]
    +\frac{K_3h_1^2}{(k+h_2)^2}+\frac{4G^2h_2^2}{(k+h_1)^2}+  12G^2\tau(\alpha_T) \alpha_{\max\{0,t-\tau(\alpha_T)\}}\\
    \leq & \Pi^k_{i=0}\left(1-\frac{K_3h_1}{2(i+h_2)} \right)V(\tilde{\vx}_0)\\
    +&\sum^{k-1}_{i=0} \Pi^k_{j=i+1}\left(1-\frac{K_3h_1}{2(j+h_2)} \right) \left(\frac{K_3h_1^2}{(i+h_2)^2}+\frac{4G^2h_2^2}{(i+h_1)^2}+12G^2\tau(\alpha_T) \alpha_{\max\{0,i-\tau(\alpha_T)\}}\right)\\
    +&\frac{K_3h_1^2}{(k+h_2)^2}+\frac{4G^2h_2^2}{(k+h_1)^2}+  12G^2\tau(\alpha_T) \alpha_{\max\{0,t-\tau(\alpha_T)\}}\\
    \leq & \exp\left(\sum^{k}_{i=0} -\frac{K_3h_1}{2(i+h_2)} \right)V(\tilde{\vx}_0)\\
    +& \sum^{k-1}_{i=0} \exp\left( \sum^k_{j=i+1} -\frac{K_3h_1}{2(j+h_2)} \right)\left(\frac{K_3h_1^2}{(i+h_2)^2}+12G^2\tau(\alpha_T) \alpha_{\max\{0,i-\tau(\alpha_T)\}} \right)\\
    +&\frac{K_3h_1^2}{(k+h_2)^2}+12G^2\tau(\alpha_T) \alpha_{\max\{0,t-\tau(\alpha_T)\}}\\
    \leq & \exp\left( -K_3h_1 \log\frac{k+h_2}{h_2} \right) V(\tilde{\vx}_0)\\
    +& \sum^{k-1}_{i=0} \exp\left(-\frac{K_3h_1}{2}\log\left(\frac{k+h_2}{i+1+h_2}\right) \right)\left(\frac{K_3h_1^2}{(i+h_2)^2}+\frac{4G^2h_2^2}{(i+h_1)^2}+12G^2\tau(\alpha_T) \alpha_{\max\{0,i-\tau(\alpha_T)\}}\right)\\
    +& \frac{K_3h_1^2}{(k+h_2)^2}+\frac{4G^2h_2^2}{(k+h_1)^2}+  12G^2\tau(\alpha_T) \alpha_{\max\{0,t-\tau(\alpha_T)\}}\\
    \leq & \frac{h_2^2}{(k+h_2)^2} V(\tilde{\vx}_0)
    +\frac{1}{(k+h_2)^2} \sum^{k-1}_{i=0} (i+1+h_2)^2\left( \frac{K_3h_1^2}{(i+h_2)^2}+\frac{4G^2h_2^2}{(i+h_1)^2}+12G^2\tau(\alpha_T) \alpha_{\max\{0,i-\tau(\alpha_T)\}} \right)\\
    +& \frac{K_3h_1^2}{(k+h_2)^2}+\frac{4G^2h_2^2}{(k+h_1)^2}+  12G^2\tau(\alpha_T) \alpha_{\max\{0,t-\tau(\alpha_T)\}}
\end{align*}


We need

\begin{align*}
    \frac{h_1}{h_2} \leq \frac{K_3}{2K_1},\;
    \frac{K_3h_1}{h_2}<1
\end{align*}
which can be achieved by \(\frac{h_1}{h_2}<\min\left\{\frac{K_3}{2K_1},\frac{1}{K_3}\right\}\). Moreover, let \(K_3h_1 = 2\), then \(2<h_2\). Then \(h_2>2\) and \(\frac{i+1+h_2}{i+h_2}<2\). Hence, we get

\begin{align*}
     V(\tilde{\vx}_k)
\leq &\frac{h_2^2}{(k+h_2)^2}V(\tilde{\vx}_0)\\
+&\frac{1}{(k+h_2)^2}\sum^{k-1}_{i=0} 4\left(K_3h_1^2+4G^2h_2^2\right)+\frac{24G^2\tau(\alpha_T)}{(k+h_2)^2}\sum^{k-1}_{i=0}(i+1+h_2)\max\left\{\frac{h_1}{h_2},\frac{h_1}{i-\tau(\alpha_T)+h_2}\right\}\\
 +& \frac{K_3h_1^2}{(k+h_2)^2}+\frac{4G^2h_2^2}{(k+h_1)^2}+  \alpha_T 12G^2\tau(\alpha_T) \alpha_{\max\{0,k-\tau(\alpha_T)\}}
\end{align*}


Note that

\begin{align*}
    &\sum^{k-1}_{i=0} (i+1+h_2) \max\left\{ \frac{h_1}{h_2}, \frac{h_1}{i-\tau(\alpha_T)+h_2} \right\}\\
    =&\sum_{i=0}^{\tau(\alpha_T)}(i+1+h_2)+\sum_{i=\tau(\alpha_T)+1}^{T-1}\\
    \leq &  (1+h_2)\frac{\tau(\alpha_T)(\tau(\alpha_T)+1+h_2)}{2}+h_1\sum^{k-1}_{i=\tau(\alpha_T)+1}\frac{i+1+h_2}{i-\tau(\alpha_T)+h_2}\\
    = & (1+h_2)\frac{\tau(\alpha_T)(\tau(\alpha_T)+1+h_2)}{2}
    + h_1 \sum^{k-1}_{i=\tau(\alpha_T)+1} \left( 1 + \frac{\tau(\alpha_T)+1}{i-\tau(\alpha_T)+h_2}\right)\\
    \leq & (1+h_2)\frac{\tau(\alpha_T)(\tau(\alpha_T)+1+h_2)}{2}
    + h_1 k +h_1 \int^{k-1}_{\tau(\alpha_T)} \log \left( t-\tau(\alpha_T) +h_2\right) dt\\
    \leq & (1+h_2)\frac{\tau(\alpha_T)(\tau(\alpha_T)+1+h_2)}{2}
    +h_1k + h_1 \log \left( \frac{T-\tau(\alpha_T)+h_2-1}{h_2} \right)
\end{align*}

Therefore, we get the result that

\begin{align*}
    V(\tilde{\vx}_T) &\leq \frac{h_2^2}{(T+h_2)^2} V(\tilde{\vx}_0)\\
     +& \frac{4(K_3h_1^2+G^2h_2^2)}{k+h_2} + \frac{24G^2h_2\tau(\alpha_T)^3}{(k+h_2)^2}+\frac{24G^2\tau(\alpha_T)}{k+h_2}
\end{align*}

\end{proof}


Consider the following : 

\begin{align}
    \bar{\mL} = \begin{bmatrix}
                    \mS_1 & \mS_2
                \end{bmatrix} 
                \begin{bmatrix}
                    \bm{0}_{q\times q} & \\
                    & \mJ
                \end{bmatrix}
                \begin{bmatrix}
                    \frac{1}{N} \mS_1^{\top}\\
                    \mS_2^{\top}
                \end{bmatrix}=\mS_2\mJ\mS_2^{\top},
\end{align}
where \(\mS_1 \in \R^{Nq \times q},\;\mS_2 \in \R^{Nq \times (N-1)q}\).

We can choose \(\bar{\mS}_1\) such that
\begin{align*}
    \mS_1 = \begin{bmatrix}
        \bm{1}_N \otimes \ve_1 & \bm{1}_N \otimes \ve_2 &\cdots \bm{1}_N \otimes \ve_q
    \end{bmatrix} \in \R^{Nq \times q},
\end{align*}
where \(\ve_i \in \R^q,,\; 1\leq i \leq q\), and choose \(\mS_2\) such that 

\begin{align*}
    \mS_2\mS_2^{\top} = \mI-\frac{1}{N}\mS_1\mS_1^{\top}.
\end{align*}


Note that

\begin{align*}
    \mS_1 \mS_1^{\top} =& \begin{bmatrix}
     \bm{1}_N \otimes \ve_1 & \bm{1}_N \otimes \ve_2 &\cdots \bm{1}_N \otimes \ve_q
    \end{bmatrix}
    \begin{bmatrix}
        (\bm{1}_N \otimes \ve_1)^{\top}\\
          (\bm{1}_N \otimes \ve_w)^{\top}\\
          \vdots\\
           (\bm{1}_N \otimes \ve_q)^{\top}
    \end{bmatrix}\\
    =& \mI_N \otimes \mI_q.
\end{align*}
Note that is has eigen-value 1.

Then, we have

\begin{align*}
    \left\| \mS_2\mS_2^{\top} \right\|_2\leq \left\| \mI - \frac{1}{N}\mS_1\mS_1^{\top}  \right\|_2
\end{align*}


Letting \(\tilde{\vtheta}=\mS_2^{\top} \vtheta,\;\tilde{\vw}=\mS_2^{\top} \vw\), and multiplying \(\mS_2^{\top}\), we get


\begin{align*}
 \tilde{\vtheta}_{k+1}&=\tilde{\vtheta}_k+\alpha_k (\mS_2^{\top}\bar{\mA}\vtheta_k- \mJ \tilde{\vtheta}_k-\mJ\tilde{\vw}_k)\\
 \tilde{\vw}_{k+1} &= \tilde{\vw}_k + \alpha_k \mJ\tilde{\vtheta}_k
\end{align*}


\begin{align*}
\begin{bmatrix}
    \tilde{\vtheta}_{k+1}\\
    \tilde{\vw}_{k+1}
\end{bmatrix}
=& \begin{bmatrix}
    \mI -\alpha_k \mJ & -\alpha_k \mJ\\
    \alpha_k \mJ & \mI 
\end{bmatrix}
\begin{bmatrix}
    \tilde{\vtheta}_k\\
    \tilde{\vw}_k
\end{bmatrix}
+ \begin{bmatrix}
    \mS_2^{\top}\bar{\mA}\vtheta_k\\
    \bm{0}_{Nq}
\end{bmatrix}\\
=& \begin{bmatrix}
    \tilde{\vtheta}_k\\
    \tilde{\vw}_k
\end{bmatrix}
+\alpha_k \begin{bmatrix}
    -\mJ & -\mJ\\
    \mJ & \bm{0}_{Nq\times Nq}
\end{bmatrix}
\begin{bmatrix}
    \tilde{\vtheta}_k\\
    \tilde{\vw}_k
\end{bmatrix}
+\alpha_k \begin{bmatrix}
    \mS_2^{\top}\bar{\mA}\vtheta_k\\
    \bm{0}_{Nq}
\end{bmatrix}.
\end{align*}


Following the recursion, we get

\begin{align*}
 & \E\left[V(\tilde{\vx}_{k+1})\right]   \\
=& \E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k) \right]+\E\left[ 2\tilde{\vx}_k^{\top}\mP \tilde{\vx}_{k+1} \right] -2 \E\left[V(\tilde{\vx}_k)\right] \\
=& \E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k) \right]+\E \left[ 2\tilde{\vx}_k^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k)\right]\\
=&\E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k ) \right]+\E\left[2\tilde{\vx}_k^{\top}\mP(\tilde{\vx}_{k+1}-\tilde{\vx}_k-\alpha_k\mH \tilde{\vx}_k) \right]+2\alpha_k \E\left[ \tilde{\vx}_k^{\top} \mP \mH \tilde{\vx}_k \right].
\end{align*}

We are ready to boound :

\begin{align*}
\tilde{\vx}_k^{\top} \begin{bmatrix}
    c\mI & \mJ\\
    \mJ & c\mI
\end{bmatrix} \begin{bmatrix}
    \mS_2^{\top}\bar{\mA}\vtheta_k\\
    \bm{0}_{Nq}
\end{bmatrix} &= \begin{bmatrix}
    \vtheta^{\top}\mS_2 & \vw_{k}^{\top}\mS_2
\end{bmatrix} \begin{bmatrix}
    c\mS_2^{\top}\bar{\mA}\vtheta_k\\
    \mJ \mS_2^{\top}\bar{\mA}\vtheta_k
\end{bmatrix}\\
&= c \vtheta_k^{\top}(\mI-\mS_1\mS_1^{\top})\bar{\mA}\vtheta_k
+\vw_k^{\top}\mS_2\mJ\mS_2^{\top}\bar{\mA}\vtheta_k
\end{align*}

Note that 
Suppose the eigen-vector is \(\begin{bmatrix}
    \vv_1\\
    \vv_2
\end{bmatrix} \in \sC^{2Nq}\), such that \(\vv:=\vv_1^*\vv_1+\vv_2^*\vv_2 =1 \).

\begin{align*}
&  \vv^* \begin{bmatrix}
    \mI -\alpha_k \mJ & -\alpha_k \mJ\\
    \alpha_k \mJ & \mI 
\end{bmatrix} \vv = \lambda\\
\iff & \vv_1^* ( \mI-\alpha_k \mJ) \vv_1 + \vv_2^*\vv_2
+ \alpha_k \vv_2^* \mJ \vv_1 -\alpha_k \vv_1^* \mJ \vv_2 = \lambda\\
\iff & 1 -\alpha_k \vv_1^* \mJ \vv_1 + \alpha_k \vv_2^* \mJ \vv_1 -\alpha_k \vv_1^* \mJ \vv_2 = \lambda 
\end{align*}






Letting 

\begin{align*}
  \begin{bmatrix}
      \frac{c}{2}\mI & \bm{0}\\
      \bm{0} & \frac{c}{2}\mI
  \end{bmatrix}   \prec \mP =\begin{bmatrix}
        c \mI & \mJ \\
        \mJ & c\mI
    \end{bmatrix} \prec
    \begin{bmatrix}
    2c\mI & \bm{0}\\
    \bm{0} & 2c \mI
    \end{bmatrix}
\end{align*}

which requires
\begin{align*}
    &\frac{c}{2}\mI -\frac{2}{c}\mJ^2 \succ 0 \iff c \geq 4\lambda_{\max}(\mJ)^2\\
    & c\mI-\frac{1}{c}\mJ^2 \succ 0 \iff c \geq \lambda_{\max}(\mJ)^2.
\end{align*}

Moreover, we have

\begin{align*}
\begin{bmatrix}
    -\mJ & \mJ\\
    -\mJ & \bm{0}_{Nq \times Nq}
\end{bmatrix}
    \begin{bmatrix}
        c \mI & \mJ \\
        \mJ & c\mI
    \end{bmatrix}
    +\begin{bmatrix}
        c \mI & \mJ \\
        \mJ & c\mI
    \end{bmatrix}
    \begin{bmatrix}
    -\mJ & -\mJ\\
    \mJ & \bm{0}_{Nq \times Nq}
\end{bmatrix}
=\begin{bmatrix}
    -2c\mJ +2 \mJ^2 & -\mJ^2\\
    -\mJ^2 & -2\mJ^2
\end{bmatrix} \prec \tau \mP
\end{align*}

% We get

% \begin{align*}
%     \left\| \tilde{\vtheta}_{k+1} \right\|_2^2 - \left\| \tilde{\vtheta}_k \right\|_2^2
%     = 2\alpha_k \tilde{\vtheta}_k^{\top}\left( \mS_2^{\top}\bar{\mA}\vtheta_k-\mJ\tilde{\vtheta}_k-\mJ\tilde{\vw}_k \right)
%     +
% \end{align*}





==> prelim/algo2.tex <==
\subsection{Algorithm 2}


Consider the following matrix:

\begin{align*}
\begin{bmatrix}
    \bar{\mA}-\bar{\mL} & \bm{0}_{Nq \times Nq} & \bm{0}_{Nq \times Nq}\\
    \bar{\mI}_{Nq} & -\bar{\mI}_{Nq}-\bar{\mL} & -\bar{\mL}\\
    \bm{0}_{Nq\times Nq} & \bar{\mL} & \bm{0}_{Nq \times Nq}
\end{bmatrix}
\begin{bmatrix}
    \bar{\vtheta}^*\\
    \bar{\vw}^*\\
    \bar{\vv}^*
\end{bmatrix}
+
\begin{bmatrix}
    \bar{\vb}\\
    \bm{0}_{Nq}\\
    \bm{0}_{Nq}
\end{bmatrix} = \bm{0}_{3Nq}.
\end{align*}

The null space vector \(\begin{bmatrix}
    \bar{\vtheta}^*\\
    \bar{\vw}^*\\
    \bar{\vv}^*
\end{bmatrix}\) should satisfy 
\begin{align*}
 (\bar{\mA}-\bar{\mL}) \bar{\vtheta}^* =& \bar{\vb}\\
 \bar{\vtheta}^*-(\mI_{Nq}+\bar{\mL})\bar{\vw}^* -\bar{\mL} \bar{\vv}^* =& \bm{0}_{Nq}\\
 \bar{\mL} \bar{\vw}^* =& \bm{0}_{Nq}
\end{align*}


Multiplying  to \( (\bm{1}_N \otimes \mI_q)^{\top}\) the first equation, we get
\begin{align*}
\frac{1}{N} \sum_{i=1}^N   \vtheta^*_i =  \mA^{-1} \left(\frac{1}{N}\sum_{i=1}^N \vb_i \right),
\end{align*}



From the last equation, we have
\begin{align*}
    \bar{\vw}^* = \bm{1}_{N} \otimes \vw ,\quad \vw \in \R^{q}.
\end{align*}



Plugging into the second equation, we get
\begin{align}
    \bar{\vtheta}^* = \bm{1}_{N}\otimes \vw + \bar{\mL} \bar{\vv}^*.
\end{align}

Multiplying \( (\bm{1}_N \otimes \mI_q)^{\top}\) to the second equation, we get

\begin{align*}
    \vw = \frac{1}{N} \sum^N_{i=1} \vtheta^*_i = \mA^{-1}\left(\frac{1}{N} \sum^N_{i=1}\vb_i \right).
\end{align*}


The transpose becomes




\begin{align*}
\begin{bmatrix}
    \bar{\mA}^{\top}-\bar{\mL} & \bar{\mI}_{Nq}  & \bm{0}_{Nq \times Nq}\\
    \bm{0}_{Nq \times Nq} & -\bar{\mI}_{Nq}-\bar{\mL} & \bar{\mL}\\
    \bm{0}_{Nq\times Nq} & -\bar{\mL} & \bm{0}_{Nq \times Nq}
\end{bmatrix}
\begin{bmatrix}
    \bar{\vtheta}^*\\
    \bar{\vw}^*\\
    \bar{\vv}^*
\end{bmatrix}
+
\begin{bmatrix}
    \bar{\vb}\\
    \bm{0}_{Nq}\\
    \bm{0}_{Nq}
\end{bmatrix} = \bm{0}_{3Nq},
\end{align*}
which should satisfy


\begin{align*}
    (\bar{\mA}^{\top}-\bar{\mL})\bar{\vtheta}^*+\bar{\vw}^* &=\bar{\vb}\\
    (-\mI_{Nq}-\bar{\mL})\bar{\vw}^*+\bar{\mL}\bar{\vv}^*&=\bm{0}_{Nq}\\
    \bar{\mL}\bar{\vw}^*&=\bm{0}_{Nq}
\end{align*}


From the last equation, we have
\begin{align*}
    \bar{\vw}^* = \bm{1}_N \otimes \vw , \quad \vw \in \R^q.
\end{align*}

Multiplying \( (\bm{1}_N \otimes \mI)^{\top} \) to the second equation, we get \(\vw = \bm{0}_q\).

Therefore the null space of \(\mE^{\top}\) is \(\begin{bmatrix} \bm{0}_Nq \\ \vv \\ \bm{0}_{Nq} \end{bmatrix}\) for \(\vv \in \mathrm{Ker}(\mL)\). Therefore, orthogonal projection on to \(\mathrm{Im}(\mA)\) is

\begin{align*}
    \mA\mA^{\dagger} \begin{bmatrix}
        \bar{\vtheta}\\
        \bar{\vw}\\
        \bar{\vv}
    \end{bmatrix}
    =\begin{bmatrix}
        \bar{\vtheta}^*\\
        \bar{\vw}^*\\
        \mathrm{Proj}(\bar{\vv})
    \end{bmatrix}
\end{align*}



==> sa.tex <==
Consider a stochastic approximation scheme:
\begin{align*}
    \vx_{k+1} = \vx_k+\alpha_k (\mA \vx_k+\bm{\eps}_k),
\end{align*}
where \(\mA\in \R^{n\times n}\) has eigenvalue of zero which is semi-simple and does not have pure imaginary
 eigenvalues. An eigenvalue is said to be semi-simple if its algebraic multiplicity and geometric multiplicity coincides. From Theorem~\ref{thm:jcf} in the Appendix, we have
\begin{align*}
    \mA:= \mT \mJ\mT^{-1},
\end{align*}
where \( \mT , \mS \in \R^{n\times n}\) , \(\mJ \in \R^{n\times n }\) is the Jordan block. Since the Jordan matrix is unique up to permutation, we can let the first \(q\) Jordan blocks as corresponding to that of zero eigenvalue of \(\mA\). Since the zero eigenvalue of \(\mA\) is semi-simple, we would have
\begin{align*}
    \mJ:= \mathrm{diag}(\bm{0}_{q\times q},\mJ_2,\mJ_3,\dots,\mJ_l ) \in \mR^{n\times n},
\end{align*}
where \( \mJ_i \in \R^{d_i\times d_i}, 2 \leq i \leq l\), and \( \sum_{i=1}^l d_i = n\) and \(d_1=q\).


Moreover, let
\begin{align*}
    \mT =  \begin{bmatrix} \mT_1 & \mT_2 & \dots & \mT_l \end{bmatrix} \in \R^{n \times n},
\end{align*}
such that \( \mT_i \in \R^{n \times d_i} ,1 \leq i \leq l\). We can see that
\begin{align*}
    \mA \mT_1 =  \mT_1 \mI_q,
\end{align*}

that is each column of \(\mT_1\) consists of linearly independent null space vectors. Moreover, we can see that first \(q\) rows of \(\mT^{-1}\) is the null space vectors of \(\mA^{\top}\).


Jordan block analysis based on has been also been studied in~\cite{panteley2020strict}. In our analysis, we prove for the general case of semi-simple eigenvalues. 


Consider 

\begin{align*}
    \mB &:= \mA-\alpha \mT_1 \mS_1^{\top} \\
        &= \mT  \mJ_B \mS^{\top}
\end{align*}
where \( \mJ_B:= \mathrm{diag}(-\alpha \mI_q,\mJ_2,\dots,\mJ_l)\). Since \(\mB\) is Hurwitz, there exists \(\mP\) such that

\begin{align*}
    \mP := \int^{\infty}_0 \exp( \mB^{\top}t ) \exp(\mB t ) dt,
\end{align*}

and

\begin{align*}
    &\mB^{\top}\mP + \mP \mB = -\mI_n \\
  \iff &   \mA^{\top}\mP + \mP\mA = -\mI_n + \alpha \left( \mS_1\mT_1^{\top}\mP + \mP \mT_1 \mS_1^{\top} \right).
\end{align*}

Suppose we are interested only in the range space solution, then
\begin{align*}
 \Tilde{\vx}_k:=   \mA\mA^{\dagger} \vx_k,
\end{align*}
we have
\begin{align*}
    \tilde{\vx}_k =\tilde{\vx}_k+\alpha_k \mA \vx_k+ \mA\mA^{\dagger}\bm{\eps}_k.
\end{align*}

Note that 
\begin{align*}
 & \E\left[V(\tilde{\vx}_{k+1})\right]   \\
=& \E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k) \right]+\E\left[ 2\tilde{\vx}_k^{\top}\mP \tilde{\vx}_{k+1} \right] -2 \E\left[V(\tilde{\vx}_k)\right] \\
=& \E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k) \right]+\E \left[ 2\tilde{\vx}_k^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k)\right]\\
=&\E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k ) \right]+\E\left[2\tilde{\vx}_k^{\top}\mP(\tilde{\vx}_{k+1}-\tilde{\vx}_k-\alpha_k\mA \tilde{\vx}_k) \right]+2\alpha_k \E\left[ \tilde{\vx}_k^{\top} \mP \mA \tilde{\vx}_k \right].
\end{align*}

Letting \(\mP = \mI\), we get

\begin{align*}
    \E[V(\tilde{\vx}_{k+1})]
    \leq -2\alpha_k \lambda_{\max}(\bar{\mA}-\bar{\mL}) \left\|\bar{\vtheta}_k \right\|_2^2
\end{align*}

Note that

\begin{align*}
2\tilde{\vx}_k^{\top}\mP \mA \tilde{\vx}_k =&\tilde{\vx}_k^{\top} (\mA^{\top}\mP+\mP\mA) \tilde{\vx}_k \\
=& - \left\lVert \tilde{\vx}_k \right\rVert_2^2
+ \alpha \tilde{\vx}_k^{\top} (\mA\mA^{\dagger})^{\top} (\mS_1\mT_1^{\top}\mP+\mP\mT_1\mS_1^{\top}) \mA\mA^{\dagger} \tilde{\vx}_k \\
=& -\left\| \tilde{\vx}_k \right\rVert^2_2.
\end{align*}

This is because column vectors of \(\mS_1\) are in \(\mathrm{Ker}(\mA^{\top})\). Therefore, we get

\begin{align*}
    \E\left[ V(\tilde{\vx}_{k+1}) \right] =&\E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k ) \right]+\E\left[2\tilde{\vx}_{k+1}\mP \alpha_k \bm{\eps}_k \right]-\left\|\tilde{\vx}_k \right\|^2_2 \\
\end{align*}


The projection operator onto \(\mathrm{Im}(\mA^{\top})\) is defined as

\begin{align*}
    \begin{bmatrix}
        \mI & \bm{0}_{d\times d}\\
        \bm{0}_{d\times d} & \mL\mL^{\dagger}
    \end{bmatrix}.
\end{align*}

Moreover, we have
\begin{align*}
 \tilde{\vx}_{k+1}-\tilde{\vx}_k - \alpha_k \mA \tilde{\vx}_k =& \mA\left( \mA^{\dagger} \vx_{k+1}-\mA^{\dagger}\vx_k-\alpha_k \mA\mA^{\dagger}\vx_k\right) \\
 =& \mA( \alpha_k \mA^{\dagger}\mA \vx_k +\alpha_k\mA^{\dagger}  \bm{\eps}_k -\alpha_k \mA\mA^{\dagger}\vx_k)\\
 =& \alpha_k \mA \mA^{\dagger}\bm{\eps}_k.
\end{align*}

Now, let us bound
\begin{align*}
    (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top} (\tilde{\vx}_{k+1}-\tilde{\vx}_k) &\leq \alpha_k^2 \left\|  \mA\tilde{\vx}_k +\mA\mA^{\dagger}\bm{\eps}_k \right\|_2^2
\end{align*}



==> sa_2.tex <==
Consider a stochastic approximation scheme:
\begin{align*}
    \vx_{k+1} = \vx_k+\alpha_k (\mA \vx_k+\bm{\eps}_k),
\end{align*}
where \(\mA\in \R^{n\times n}\) has eigenvalue of zero which is semi-simple and does not have pure imaginary
 eigenvalues. An eigenvalue is said to be semi-simple if its algebraic multiplicity and geometric multiplicity coincides. From Theorem~\ref{thm:jcf} in the Appendix, we have
\begin{align*}
    \mA:= \mT \mJ\mT^{-1},
\end{align*}
where \( \mT , \mS \in \R^{n\times n}\) , \(\mJ \in \R^{n\times n }\) is the Jordan block. Since the Jordan matrix is unique up to permutation, we can let the first \(q\) Jordan blocks as corresponding to that of zero eigenvalue of \(\mA\). Since the zero eigenvalue of \(\mA\) is semi-simple, we would have
\begin{align*}
    \mJ:= \mathrm{diag}(\bm{0}_{q\times q},\mJ_2,\mJ_3,\dots,\mJ_l ) \in \mR^{n\times n},
\end{align*}
where \( \mJ_i \in \R^{d_i\times d_i}, 2 \leq i \leq l\), and \( \sum_{i=1}^l d_i = n\) and \(d_1=q\).


Moreover, let
\begin{align*}
    \mT =  \begin{bmatrix} \mT_1 & \mT_2 & \dots & \mT_l \end{bmatrix} \in \R^{n \times n},
\end{align*}
such that \( \mT_i \in \R^{n \times d_i} ,1 \leq i \leq l\). We can see that
\begin{align*}
    \mA \mT_1 =  \mT_1 \mI_q,
\end{align*}

that is each column of \(\mT_1\) consists of linearly independent null space vectors. Moreover, we can see that first \(q\) rows of \(\mT^{-1}\) is the null space vectors of \(\mA^{\top}\).


Jordan block analysis based on has been also been studied in~\cite{panteley2020strict}. In our analysis, we prove for the general case of semi-simple eigenvalues. 


Consider 

\begin{align*}
    \mB &:= \mA-\alpha \mT_1 \mS_1^{\top} \\
        &= \mT  \mJ_B \mS^{\top},
\end{align*}
where \( \mJ_B:= \mathrm{diag}(-\alpha \mI_q,\mJ_2,\dots,\mJ_l)\). Since \(\mB\) is Hurwitz, there exists \(\mP\) such that

\begin{align*}
    \mP := \int^{\infty}_0 \exp( \mB^{\top}t ) \exp(\mB t ) dt,
\end{align*}

and

\begin{align*}
    &\mB^{\top}\mP + \mP \mB = -\mI_n \\
  \iff &   \mA^{\top}\mP + \mP\mA = -\mI_n + \alpha \left( \mS_1\mT_1^{\top}\mP + \mP \mT_1 \mS_1^{\top} \right).
\end{align*}

Suppose we are interested only in the range space solution, then
\begin{align*}
 \Tilde{\vx}_k:=   \mA\mA^{\dagger} \vx_k,
\end{align*}
we have
\begin{align*}
    \tilde{\vx}_k =\tilde{\vx}_k+\alpha_k \mA \vx_k+ \mA\mA^{\dagger}\bm{\eps}_k.
\end{align*}

Note that 
\begin{align}
 & \E\left[V(\tilde{\vx}_{k+1})\right] \nonumber   \\
=& \E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k) \right]+\E\left[ 2\tilde{\vx}_k^{\top}\mP \tilde{\vx}_{k+1} \right] -2 \E\left[V(\tilde{\vx}_k)\right] \nonumber \\
=& \E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k) \right]+\E \left[ 2\tilde{\vx}_k^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k)\right] \nonumber\\
=&\E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k ) \right]+\E\left[2\tilde{\vx}_k^{\top}\mP(\tilde{\vx}_{k+1}-\tilde{\vx}_k-\alpha_k\mA \tilde{\vx}_k) \right]+2\alpha_k \E\left[ \tilde{\vx}_k^{\top} \mP \mA \tilde{\vx}_k \right].  \nonumber
\end{align}

% Letting \(\mP = \begin{bmatrix}
%     \mI_{ Nq \times Nq } & \bm{0}_{Nq\times Nq}\\
%     \bm{0}_{Nq\times Nq} & \bm{0}_{Nq\times Nq}
% \end{bmatrix}\), we get

% \begin{align*}
%     \E[V(\tilde{\vx}_{k+1})]
%     \leq -2\alpha_k \lambda_{\max}(\bar{\mA}-\bar{\mL}) \left\|\bar{\vtheta}_k \right\|_2^2
% \end{align*}

% Note that

% \begin{align*}
% 2\tilde{\vx}_k^{\top}\mP \bar{\mA} \tilde{\vx}_k =&\tilde{\vx}_k^{\top} \begin{bmatrix}
%     -\bar{\mA}-\bar{\mA}^{\top}-2\bar{\mL} & \bm{0}_{Nq\times Nq}\\
%     \bm{0}_{Nq\times Nq} & \bm{0}_{Nq\times Nq}
% \end{bmatrix} \tilde{\vx}_k
% \end{align*}

% This is because column vectors of \(\mS_1\) are in \(\mathrm{Ker}(\mA^{\top})\). Therefore, we get

\begin{align}
    \E\left[ V(\tilde{\vx}_{k+1}) \right] =&\E\left[ (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k ) \right]+\E\left[2\tilde{\vx}_{k+1}\mP \alpha_k \bm{\eps}_k \right]-\left\|\tilde{\vx}_k \right\|^2_2 \label{eq:V}
\end{align}


The projection operator onto \(\mathrm{Im}(\mA^{\top})\) is defined as

\begin{align*}
  \mA\mA^{\dagger} =   \begin{bmatrix}
        \mI & \bm{0}_{d\times d}\\
        \bm{0}_{d\times d} & \mL\mL^{\dagger}
    \end{bmatrix}.
\end{align*}

Moreover, we have
\begin{align*}
 \tilde{\vx}_{k+1}-\tilde{\vx}_k - \alpha_k \mA \tilde{\vx}_k =& \mA\left( \mA^{\dagger} \vx_{k+1}-\mA^{\dagger}\vx_k-\alpha_k \mA\mA^{\dagger}\vx_k\right) \\
 =& \mA( \alpha_k \mA^{\dagger}\mA \vx_k +\alpha_k\mA^{\dagger}  \bm{\eps}_k -\alpha_k \mA\mA^{\dagger}\vx_k)\\
 =& \alpha_k \mA \mA^{\dagger}\bm{\eps}_k.
\end{align*}

Now, let us bound
\begin{align*}
    (\tilde{\vx}_{k+1}-\tilde{\vx}_k)^{\top}\mP (\tilde{\vx}_{k+1}-\tilde{\vx}_k) &\leq \alpha_k^2 \lambda_{\max}(\mP) \left\|  \mA\tilde{\vx}_k +\mA\mA^{\dagger}\bm{\eps}_k \right\|_2^2\\
    &\leq 2\alpha_k^2 \lambda_{\max}(\mP) \sigma_{\max}(\mA)^2 \left\|\tilde{\vx}_k \right\|_2^2
    +2\alpha_k^2 C_1\left\| \bar{\vtheta}_k \right\|_2^2+\alpha_k^2C_2\\
    &\leq (\lambda_{\max}(\mP) \sigma_{\max}(\mA)^2+C_1)\alpha_k^2\left\| \tilde{\vx}_k \right\|^2_2+\alpha_k^2C_2\\
    &\leq K_1\alpha_k^2 V(\tilde{\vx}_k)+\alpha_k^2K_2
\end{align*}

Plugging into~(\ref{eq:V}), we get

\begin{align*}
     &\E[V(\tilde{\vx}_{k+1})-\E[V(\tilde{\vx}_k)]] \\
    \leq & K_1 \alpha_k^2 V( \tilde{\vx}_k)+\alpha_k^2 K_2
    + 2\alpha_k\E[\tilde{\vx}_{k+1}^{\top}\mP\bm{\eps}(\bar{\vx}_k,\bar{\xi}_k)]-K_3\alpha_k V(\tilde{\vx}_k)
\end{align*}


If the chain is i.i.d., it becomes
\begin{align*}
    \E[V(\tilde{\vx}_{k+1})] \leq \left( 1+K_1\alpha_k^2-K_3\alpha_k \right) \E[V(\tilde{\vx}_k)]+\alpha_k^2 K_2
\end{align*}

First we should have \(K_1\alpha_k^2-K_3\alpha_k\leq -\frac{K_3}{2}\alpha_k\), which leads to \(\alpha_k \leq \frac{K_3}{2K_1}\). Hence, we get

\begin{align*}
    \E[V(\tilde{\vx}_{k+1})] \leq \left(1-\frac{K_3}{2}\alpha_k\right) \E[V(\tilde{\vx}_k)]+\alpha_k^2 K_2.
\end{align*}

Suppose we select diminishing step size : 
\begin{align*}
    \alpha_k := \frac{h_1}{k+h_2},
\end{align*}

we have

\begin{align*}
    \E[V(\tilde{\vx}_{k+1})] \leq \left(1-\frac{K_3h_1}{k+h_2} \right)\E[V(\tilde{\vx}_k)]+\frac{K_3h_1^2}{(k+h_2)^2}
\end{align*}
